HoloFusion: Towards Photo-realistic 3D Generative Modeling

Diffusion-based image generators can now produce high-quality and diverse samples, but their success has yet to fully translate to 3D generation: existing diffusion methods can either generate low-resolution but 3D consistent outputs, or detailed 2D views of 3D objects but with potential structural defects and lacking view consistency or realism. We present HoloFusion, a method that combines the best of these approaches to produce high-fidelity, plausible, and diverse 3D samples while learning from a collection of multi-view 2D images only. The method first generates coarse 3D samples using a variant of the recently proposed HoloDiffusion generator. Then, it independently renders and upsamples a large number of views of the coarse 3D model, super-resolves them to add detail, and distills those into a single, high-fidelity implicit 3D representation, which also ensures view consistency of the final renders. The super-resolution network is trained as an integral part of HoloFusion, end-to-end, and the final distillation uses a new sampling scheme to capture the space of super-resolved signals. We compare our method against existing baselines, including DreamFusion, Get3D, EG3D, and HoloDiffusion, and achieve, to the best of our knowledge, the most realistic results on the challenging CO3Dv2 dataset.

==> src/suppl_body.tex <==
 \section{Views2Voxel-grid unprojection mechanism}
\newcommand{\real}{\mathbb{R}}
\newcommand{\bp}{\mathbf{p}}
Given a training video $s$ containing frames $I_j$, we obtain the auxiliary grid $\bar V \in \real^{d \times S \times S \times S}$
of auxiliary features $\bar V_{:mno} \in [-1, 1]^{d}$ by using the following procedure.
The values $m,n,o \in \mathbb{N}$ index the 3D grid of size [$S \times S \times S$].
We first project the 3D coordinate $\bp^{\bar V}_{mno}$ of each grid vertex (corner) $(m,n,o)$  to every video frame $I_j$ and sample corresponding 2D image features.
The 2D image features $f_{mno}^{j}$ are obtained using a frozen ResNet-32 encoder~\cite{he16deep} $E(I_j)$.
We use bilinear interpolation for sampling continuous values and use zero-features for projected points that lie outside the image region on the 3D image plane.
Thus, we obtain $N_\text{frames}$ feature-vectors (corresponding to each frame in the video) for each grid element of the voxel-grid.
We accumulate these features using the accumulator MLP $\mathcal{A}_{acc}$.
The accumulator $\mathcal{A}_{acc}$ takes as input $[f_{mno}^{j}; v^j]$, where $[~;~]$ denotes concatenation and $v^j$ corresponds to the viewing direction of the camera center of $j^{\text{th}}$ frame, and outputs $[\sigma^j_{mno}; {f'}_{mno}^{j}]$.
Here, the value $\sigma^j$ corresponds to a weight for $j^\text{th}$ feature vector and $f'^j$ is an MLP transformed version of the input feature vector.
Lastly, we compute the aggregated feature vector (for each of the voxel grid centers) as a weighted sum of the transformed features:
\begin{equation}
    \bar V_{:mno} = F_{mno} = \sum_{j} \sigma^j_{mno} {f'}_{mno}^{j}.
\end{equation}

% \section{HoloDiffusion anonymous copy}
% An anonymous copy of the CVPR 2023 accepted paper titled \textbf{``HoloDiffusion: Training a 3D diffusion model using 2D Images''} is provided in the supplementary material along with this pdf. Please find the copy enclosed in the zip archive.

\section{\method{Stable-DreamFusion} baseline details}
\paragraph{Implementation  details}  Since no code is available for either of the two 2D diffusion distillation works, DreamFusion \cite{poole2022dreamfusion} and Magic3D \cite{lin2022magic3d}, we resort to using the open-source implementation provided by the GitHub user \href{https://github.com/ashawkey}{ashawkey} titled \href{https://github.com/ashawkey/stable-dreamfusion}{\method{Stable-DreamFusion}} \cite{stable-dreamfusion}. The differences between the implementation and the aforementioned research works are as follows:
\begin{enumerate}
    \item While DreamFusion uses the Imagen \cite{ho2022imagen} diffusion model, and Magic3D uses a combination of Ediff-I \cite{balaji2022ediffi} and StableDiffusion \cite{rombach2021stablediffusion}, the implementation only uses StableDiffusion since Imagen and Ediff-I models are unavilable.

    \item Since the used diffusion network of StableDiffusion performs diffusion in the latent-space, the implementation applies the SDS loss in the latent space and backpropagates the SDS gradients through the perceptual encoder.
    
    \item The DIP generator (backbone) is implemented as a vanilla NeRF \cite{mildenhall20nerf:} as opposed to the Mip-NeRF \cite{barron2021mip} version as used by DreamFusion. 
\end{enumerate}

\paragraph{Prompt builder} 
We use a simple procedure to generate the prompts used for distilling the samples from the \method{Stable-DreamFusion} \cite{stable-dreamfusion} baseline. We first start by defining three python lists (aka. Prompt Builder Ingredients), viz. \texttt{objects}, \texttt{modifiers}, and \texttt{colors}. The \texttt{objects} list is set to verbose names of the categories from the Co3Dv2 \cite{reizenstein21common} which we used in our experiments. \cref{tab:prompt-ingredients} describes the values for the ingredient lists in full. Then we generate a shuffled list of all prompts by taking a full outer-product of the ingredients and ensuring correct grammar.  
% using the \texttt{get\_all\_prompts} function as provided in the code listing in \cref{fig:prompt-building-code}. 
Some of the generated final prompts are given in the \cref{tab:sample_prompts}.

% \begin{code}[The code snippet used to populate the prompts used to distill 3D radiance fields using the stable-dreamfusion \cite{stable-dreamfusion} implementation. Please refer the \cref{tab:prompt_ingredients} for the values of \texttt{modifiers}, \texttt{colors}, and \texttt{objects}. \label{fig:prompt-building-code}]
% def a_or_an(char: str) -> str:
%     return "an" if char in "aeiou" else "a"

% def get_all_prompts(modifiers: List[str], colors: List[str], objects: List[str]) -> List[str]:
%     all_prompts = []
%     for modifier in [""] + modifiers:
%         for color in [""] + colors:
%             for obj in objects:
%                 if modifier:
%                     prompt = f"{a_or_an(modifier[0])} {modifier}"
%                     if prompt.endswith("of"):
%                         # an additional "a/an" is needed for modifiers ending with "of"
%                         # for instance "a dslr photo of a green apple"
%                         if color:
%                             prompt += f"{a_or_an(color[0])} {color}"
%                         else:
%                             prompt += f" {a_or_an(obj[0])}"
%                 else:
%                     if color:
%                         prompt = f"{a_or_an(color[0])} {color}"
%                     else:
%                         prompt = a_or_an(obj[0])
%                 prompt += f" {obj}"
%                 all_prompts.append(prompt)
%     random.shuffle(all_prompts)
%     return all_prompts
% \end{code}


\begin{table*}
\centering
\caption{The values of the builder ingredients \texttt{objects}, \texttt{modifiers}, and \texttt{colors} used for generating the prompts for stable-dreamfusion \cite{stable-dreamfusion}. \label{tab:prompt-ingredients}}
\begin{tabular}{|l|p{0.7\linewidth}|}
\hline
\textbf{Prompt Builder Ingredient} & \textbf{Values used}  \\
\hline
\texttt{objects}   &  ``apple", ``water hydrant", ``teddy bear", ``donut" \\
\hline
\texttt{modifiers} & ``unreal render of", ``zoomed out unreal render of", ``wide angle zoomed out unreal render of", ``dslr photo of", ``zoomed out dslr photo of", ``wide angle zoomed out dslr photo of", ``plastic", ``metallic", ``wooden", ``furry" \\
\hline
\texttt{colors}    & ``red", ``green", ``blue", ``yellow",  ``orange", ``brown", ``pink", ``purple", ``cyan", ``magenta", ``sky blue", ``baby blue", ``crimson", ``lime", ``teal", ``violet", ``sea green", ``dusk", ``gold", ``silver" \\
\hline
\end{tabular}
\end{table*}


\begin{table}
\centering
\caption{A sampling of the prompts generated after running the prompt-building process. \label{tab:sample_prompts}}
\begin{tabular}{|p{1.0\linewidth}|}
\hline
\textbf{Sample prompts} \\
\hline
 ``\texttt{a plastic teddy bear}'', \\
 ``\texttt{a zoomed out unreal render of a water hydrant}'', \\
 ``\texttt{a wide angle zoomed out unreal render of a dusk donut}'', \\
 ``\texttt{a dslr photo of a water hydrant}'', \\
 ``\texttt{a plastic apple}'', \\
 ``\texttt{a sea green apple}'', \\
 ``\texttt{an unreal render of a red apple}'', \\
 ``\texttt{an unreal render of a silver donut}'', \\
 ``\texttt{a baby blue water hydrant}'', \\
 ``\texttt{a metallic donut}'' \\
\hline
\end{tabular}
\end{table}

% \section{Additional qualitative results}
% We provide a zip containing an  html-page that can be viewed \textit{locally} using any browser (we recommend firefox). The html shows supplementary videos of our results. In order to view the webpage, please unzip the zip file provided as a part of the supplementary material and open the \texttt{focussed\_results.html}.


